FedDG: Federated Domain Generalization on Medical Image Segmentation via Episodic Learning in Continuous Frequency Space

Federated learning allows distributed medical institutions to collaboratively learn a shared prediction model with privacy protection. While at clinical deployment, the models trained in federated learning can still suffer from performance drop when applied to completely unseen hospitals outside the federation. In this paper, we point out and solve a novel problem setting of federated domain generalization (FedDG), which aims to learn a federated model from multiple distributed source domains such that it can directly generalize to unseen target domains. We present a novel approach, named as Episodic Learning in Continuous Frequency Space (ELCFS), for this problem by enabling each client to exploit multi-source data distributions under the challenging constraint of data decentralization. Our approach transmits the distribution information across clients in a privacy-protecting way through an effective continuous frequency space interpolation mechanism. With the transferred multi-source distributions, we further carefully design a boundary-oriented episodic learning paradigm to expose the local learning to domain distribution shifts and particularly meet the challenges of model generalization in medical image segmentation scenario. The effectiveness of our method is demonstrated with superior performance over state-of-the-arts and in-depth ablation experiments on two medical image segmentation tasks. The code is available at "https://github.com/liuquande/FedDG-ELCFS".

==> episodic.tex <==

\subsection{Boundary-oriented Episodic Learning}
% \subsection{Ambiguity-driven Meta-learning}
% \subsubsection{Meta-learning towards generalizability}
\label{meta}
% \textbf{Local meta learning:}
\textbf{Episodic learning at local client:}
The generated continuous multi-source distributions lay foundation for each client to learn generalizable local parameters, but this requires careful design of the local training. 
% but this is not naturally happened. 
% In this regard, we further formulate the local training as an episodic meta-learning scheme to expose the model optimization to domain shift by splitting the training data as meta-train and meta-test.
We formulate the local training as an episodic meta-learning scheme, which learns generalizable model parameters by simulating train/test domain shift during the model training process.
% The simulated distributions lays foundation to optimize the local parameters towards domain invariance, but that is not naturally happened. To effectively exploit the simulated distributions, we formulate the local training as a meta-learning scheme~\cite{finn2017model}, to promote generalizable optimization by simulating the real-wolrd domain shift in the learning process.
Specifically, in each iteration, we consider the raw input $x_i^k$ as meta-train and its multiple transformed counterparts $t_i^k=\{x_i^{k\rightarrow n}\}_{n \neq k}$  as meta-test presenting distribution shift. The meta learning scheme can then be divided into two steps. First, the model parameters $\theta^k$ are updated on meta-train
with segmentation Dice loss $\mathcal{L}_{seg}$:
\begin{equation}
\small
\hat{\theta}^{k}= \theta^k - \alpha \nabla_{\theta^k}\mathcal{L}_{seg}(x_i^k; \theta^k),
\label{innerloop}
\end{equation}
where $\alpha$ is the meta learning rate for the inner-loop update. Second, a meta-update is performed to virtually evaluate the updated parameters on the held-out transformed data $t_i^k$ with meta-objective $\mathcal{L}_{meta}$. Crucially, this objective is computed with the updated parameters $\hat{\theta}^{k}$, but optimized w.r.t the original parameters $\theta^k$. Such optimization paradigm aims to train the model such that its learning on source domain can further exhibit certain properties that we desire in unseen domains, 
which are quantified by $\mathcal{L}_{meta}$.


\textbf{Boundary-oriented meta optimization:} 
Next, we define $\mathcal{L}_{meta}$ with considering specific challenges in medical image segmentation scenarios. Particularly, it is observed that the performance drop of medical image segmenation at unseen domains mainly comes from the ambiguous boundary regions of anatomies. In this regard, how to regularize the model towards domain-invariant discrimination around the the boundary area is especially important for the generalization problem in medical image segmentation. To achieve this, we propose a new boundary-oriented objective $\mathcal{L}_{boundary}$ into meta-optimization, to explicitly promote the clustering of boundary-related and background-related embeddings regardless of distributions while reducing their overlaps.

% extract discriminative representations around the boundary regions that are domain-invariant, such 
% We thus aim to guide the model to learn domain-invariant discrimination with reduced class ambiguity at the boundary area. 
% To achieve that, the embeddings of the same class should lie close to each other regardless of the data domains while the embeddings of different classes should be away from each other to be better separated.
% We therefore introduce an ambiguous region oriented regularization objective into the meta optimization process, to explicitly encourage the intra-class compactness and inter-class separation of the boundary and background clusters.

% Motivated by this, the model is expect to enhance the discrimination ability for the ambiguous regions at distribution shift, so that the anatomy structure can still be accurately delineated at unseen domain.  To achieve that, we introduce a new meta objective to facilitate domain-invariant discrimination for the ambiguity around boundary regions, by explicitly regularizing the model to capture discriminative boundary and background embeddings that cluster regardless of domains. 


% expect the model to well delineate the anatomy boundary at unseen domains. This, however, is challenging when distribution shift is encountered, and we observe that the performance drop at unseen domains mainly comes from the ambiguous boundary regions. In this regard, we introduce a new boundary enhancement meta objective to improve the boundary delineation at distribution shift, by explicitly regularizing the model to capture discriminative boundary and background embeddings that cluster regardless of domains. 
% Particularly, we expect the model can well delineate the boundary of anatomies at unseen domains, which is a critical problem in medical image segmentation~\cite{lee2020structure}. This, however, is challenging when distribution shift is encountered, and we observe that the performance drop at unseen domains outside federations mainly comes from the ambiguous boundary regions. Therefore, in addition to the segmentation objective, we further propose a boundary enhancement objective in the meta optimization, to explicitly promote the discrimination and domain invariance for embeddings around the boundary regions.
% the prototpe representations~\cite{snell2017prototypical} (i.g., mean of class features) for the

Specifically, given image $x_i^k$ with segmentation label $y_i^k$,  we first extract its binary boundary mask $y_{i\_bd}^k$ and background mask $y_{i\_bg}^k$ with morphological operations on $y_i^k$.
% To extract their embeddings around the ambiguous boundary, we first perform morphological operations on $y_i^k$ to obtain their binary boundary mask $y_{i\_bd}^k$  and background mask $y_{i\_bg}^k$. 
Notably, the mask $y_{i\_bg}^k$ only contain background pixels around the anatomy boundary, as we expect to enhance the discrimination for features around to the ambigious boundary regions. Let $Z^l$ denote the activation map extracted from layer $l$, which is interpolated with  bilinear interpolation to keep consistent dimensions as $y_i^k$. Then the boundary-related and background-related embeddings of $x_i^k$ can be extracted from $Z_i^l$ with masked average pooling over $y_{i\_bd}^k$ and $y_{i\_bg}^k$ as:
% \begin{equation}
% p_{i\_bd}^{[\cdot]}=\frac{\sum < F_i^{[\cdot]}, y_{i\_bd}^k>}{\sum y_{i\_bd}^k};
% p_{i\_bg}^{[\cdot]}=\frac{\sum < F_i^{[\cdot]}, y_{i\_bg}^k>}{\sum y_{i\_bg}^k}
% \end{equation}
\begin{equation}
\small
h_{i\_bd}=\frac{\sum < Z^l_i, y_{i\_bd}^k>}{\sum y_{i\_bd}^k};
h_{i\_bg}=\frac{\sum < Z^l_i, y_{i\_bg}^k>}{\sum y_{i\_bg}^k},
\end{equation}
where $\langle\cdot,\cdot\rangle$ denote the dot product operation. The produced $h_{i\_bd}$ and $h_{i\_bg}$ are single-dimensional vectors, representing the region-level features of boundary and background pixels around the ambiguous boundary regions.
% $[\cdot] \in [k, \{k\rightarrow -k\}]$. 
By further performing the same operation for $K-1$ transormed images $t_i^k=\{x_i^{k\to n}\}_{n\neq k}$, we accordingly obtain together $K$ boundary-related embeddings and $K$ background-related embeddings, each of which corresponds to features extracted from a certain distribution [$\mathcal{X}_1, \cdots, \mathcal{X}_K$]. 

To promote the domain-independent discrimination of the ambiguous-region features, we expect that the boundary and background-related embeddings should be respectively projected to a compact space regardless of distributions, but further pushed away from each other. 
% Motivated by this objective, we perform contrastive learning~\cite{chen2020simple} within the $2 \times K$ embeddings.
% There has been various popular loss functions designed to promote the class-specific clusters while reducing their overlap
Here, we adopt the well-established  InfoNCE~\cite{chen2020simple} objective to achieve this goal, which works in a way to regularize the angular space distance between pair of features  to promote class-specific clusters while reducing cluster overlaps. 
% The contrastive loss function for a positive pair of examples $(p_{i\_bd}^k,p_{i\_bd}^{k\to n})$ is defined as:
% \begin{equation}
% \mathcal{L}_{con}(p_{i\_bd}^k,p_{i\_bd}^{k\to n})=-log\frac{exp(p_{i\_bd}^k \odot p_{i\_bd}^{k\to n} / \tau)}{\sum_{q\in \Omega} exp(p_{i\_bd}^k \odot q / \tau)},
% \end{equation}
% where $\Omega$ denotes the set $\{p_{i\_bg}^k,\{p_{i\_bg}^{k\to n}\}_{n\neq k}\}$;
% $\odot$ denotes the cosine similarity: $a \odot b = \frac{\langle a,b \rangle}{||a||_2||b||_2}$;
% $\tau$ denotes the temperature parameter.
Denote ($h_l, h_m$) as a pair of embeddings, which is a positive pair if $h_l$ and $h_m$ are of the same class (both boundary-related or background-related) and otherwise negative pair. 
% We then define the contrastive loss for each positive pair ($h_l, h_m$) within the $2 \times K$ embeddings as follows:  
In our case, the InfoNCE loss is defined over each positive pair ($h_l, h_m$) within the $2 \times K$ region-level embeddings as:
\begin{equation}
\small
\ell(h_l,h_m)=-log\frac{exp(h_l \odot h_m / \tau)}{\sum_{q=1}^{2K} \mathbb{F}(h_l, q)\cdot exp(h_l \odot h_m / \tau)},
\end{equation}
where $\odot$ denote the cosine similarity: $a \odot b = \frac{\langle a,b \rangle}{||a||_2||b||_2}$; the value of $\mathbb{F}(h_l, q)$ is 0 and 1 for positive and negative pair respectively; $\tau$ denotes the temperature parameter. The final loss $\mathcal{L}_{boundary}$ is the average of $\ell$ over all positive pairs:
%The final loss of the ambiguity enhancement objective $\mathcal{L}_{ambiguity}$ is the average of $\mathcal{L}_{con}$ over all positive pairs.
\begin{equation}
\small
\mathcal{L}_{boundary}=\sum_{l=1}^{2K}\sum_{m=l+1}^{2K}\mathbb{F}(h_l, h_m)\cdot \ell (h_l, h_m) / (B(K,2)\times2),
\end{equation}
where $B(K,2)$ is the number of combinations.


% Given that directly minimizing their feature distance might be a too strict constraint, we perform contrastive learning~\cite{oord2018representation} to achieve that goal. Specifically, given a positive pair ($m$, $n$) of the same type from the $2 \times K$ prototypes, their contrastive loss is defined as follows:  
% \begin{equation}
% \mathcal{L}_{con}(m,n)=-log\frac{exp(m \odot n / \tau)}{\sum_{q=0}^{2K-1} \mathbb{F}(m, q)\cdot exp(m \odot n / \tau)}
% \end{equation}
% where $\odot$ denote the cosine similarity: $a \odot b = \frac{\langle a,b \rangle}{||a||_2||b||_2}$; the value of $\mathbb{F}(m,q)$ is 0 and 1 for positive and negative pair respectively; $\tau$ demote the temperature parameter. The final boundary enhancement objective $\mathcal{L}_{boundary}$ is the average of $\mathcal{L}_{con}$ over all positive pairs within the $2 \times K$ prototypes.

\textbf{Overall local learning objective:}
In our case, the overall meta objective is composed of the segmentation dice loss $\mathcal{L}_{seg}$ and the boundary-oriented objective $\mathcal{L}_{boundary}$ as:
% \begin{equation}
% \mathcal{L}_{meta} = \mathcal{L}_{seg}(x_i^{k\rightarrow -k};(\theta^k)') + \gamma\mathcal{L}_{ambiguity}(x_i^k, x_i^{k\rightarrow -k};(\theta^k)')
% \end{equation}
\begin{equation}
\mathcal{L}_{meta} = \mathcal{L}_{seg}(t_i^k;\hat{\theta}^{k}) + \gamma\mathcal{L}_{boundary}(x_i^k, t_i^k;\hat{\theta}^{k}),
\end{equation}
where $\hat{\theta}^k$ is the updated parameter from Eq.~\ref{innerloop}, $\gamma$ is a hyper-parameter to balance the two objectives. Finally, both the inner loop objective and  meta objective will be optimized together with respect to the original parameter $\theta^k$ as:
\begin{equation}
\mathop{\arg\min}_{\theta^k} \mathcal{L}_{seg}(x_i^k; \theta^k) + \mathcal{L}_{meta}(x_i^k, t_i^k;\hat{\theta}^{k}).
\label{eq:meta}
\end{equation}
In a federated round, once the local learning is finished, the local parameters $\theta^k$ from all clients will be aggregated with the FedAvg algorithm to update the global model.  
